An Early Experience with Confidential Computing Architecture for On-Device Model Protection

Deploying machine learning (ML) models on user devices can improve privacy (by keeping data local) and reduce inference latency. Trusted Execution Environments (TEEs) are a practical solution for protecting proprietary models, yet existing TEE solutions have architectural constraints that hinder on-device model deployment. Arm Confidential Computing Architecture (CCA), a new Arm extension, addresses several of these limitations and shows promise as a secure platform for on-device ML. In this paper, we evaluate the performance-privacy trade-offs of deploying models within CCA, highlighting its potential to enable confidential and efficient ML applications. Our evaluations show that CCA can achieve an overhead of, at most, 22% in running models of different sizes and applications, including image classification, voice recognition, and chat assistants. This performance overhead comes with privacy benefits; for example, our framework can successfully protect the model against membership inference attack by an 8.3% reduction in the adversary's success rate. To support further research and early adoption, we make our code and methodology publicly available.

==> parts/Experimental_setup.tex <==











 



==> parts/motivation.tex <==
\SA{Integrate this part}

\iffalse
Model providers desire model privacy as their models might be proprietary; providers do not want to expose any information about their models or training data to external parties such as other (potentially competing) model providers, the end-user, or malicious actors \cite{siby2024guarantee}. 
%
Model providers also require model verifiability, to ensure that their models exhibit the expected behavior and have not been tampered with. 
%
Leaked or modified models, especially in security-critical applications such as banking or medical services, can result in harm to the end-user \eg identity theft or exposure of personal information~\cite{sun2021mind}.
%
Current on-device TEE architectures are unable to meet the necessary security and functionality requirements. 
More specifically, their limited memory \cite{mo2022sok} and dangerous high privilege \cite{cerdeira2020sok} severely hinder their usage in deployment of on-device models. The introduction of CCA presents new opportunities by providing a memory-unlimited and de-privileged TEE, called realm. The architecture also offers formally verified guarantees of confidentiality and integrity—making it the first confidential computing architecture to do so \cite{li2022design,fox2023verification}. 
\fi
Given that Arm is the dominant architecture in mobile and edge devices, and is projected to significantly expand its market share in personal computers \cite{armdesktop}, we anticipate CCA's widespread deployment. These key features encourage us to evaluate the architecture, prior to its adoption on end-devices. Within a realm,  we can go beyond evaluating small models deployed in on-device TEEs (\eg in \cite{bayerl2020offline, zhang2024tsdp, xie2024memory}) to large language models (LLMs).

Our initial evaluations within FVP revealed two key issues within the default settings: (1) running workloads within a realm VM incurs a significant overhead compared to executing them in a NW VM, and (2) there is inconsistency in the results across multiple runs of the same experiment within a realm VM. These issues have also been recognized by the community \cite{githubtimer,armcommunity}, which is not surprising given that Arm CCA is still in its developmental stages. Addressing these problems is particularly critical in our case, as we run much heavier workloads within the realm compared to previous works \cite{sridhara2024acai,wang2024cage,siby2024guarantee}, and any inconsistency could significantly impact our results. Furthermore, resolving these issues or identifying an optimal configuration could be valuable not only for our work but also for the broader community and CCA developers. 
%

Another question that may arise is whether the security advantages of deploying a model within a realm justify the associated overhead, particularly given that end-devices are typically resource-constrained. To address this, we demonstrate the protections offered by Arm CCA through privacy-stealing attacks targeting the dataset on which the model is trained. This serves as a showcase of the enhanced security provided by CCA, helping to evaluate whether the overhead is worth the trade-off for improved privacy protection. However, the advantages of CCA extend beyond this evaluation by also safeguarding the model against tampering by adversaries and reducing the Trusted Computing Base (TCB) through its architectural design.








